Design, Implementation, and Evaluation of Blockchain-Based Trusted Achievement Record System for Students in Higher Education

With a growing number of institutions involved in the global education market, it has become increasingly challenging to verify the authenticity of academic achievements such as CVs and diplomas. Blockchain is an enabling technology that can play a key role in solving this problem. This study introduces a blockchain-based achievement record system that produces a verifiable record of achievements. The proposed system aims to facilitate the process of authentication and validation of certificates reliably, easily, and quickly, leveraging the unique capabilities offered through Blockchain technology (public Ethereum Blockchain) and smart contracts. We present the design and implementation of the system and its components and tools. We then evaluate the system through a number of studies to measure the system's usability, effectiveness, performance, and cost. A System Usability Scale (SUS) test gave a scale of 77.1. Through a literature survey, we demonstrate that this system is a significant improvement on legacy systems, being both more user-friendly and more efficient. We also conduct a detailed cost analysis and discuss the positives and limitations of alternative blockchain solutions.

==> table.tex <==
\newpage
\begin{table}[p] 
\caption{Summary Comparison of Various Solutions.}
\label{tab:Summary Comparison of Various Solutions.}
\begin{tabular}{lcllllll}
\hline
              & \multicolumn{7}{c}{Features} \\ \hline
 & \multicolumn{1}{l}{Accreditation} & VERIFICATION & PRIVACY & Transparency & USER& Accessibility & Sharing \\
 
  &  &  &  &  & EXPERIENCE &  & Record \\\hline
OpenBadge     & $\bullet$  & $\otimes$ & $\bullet$  & $\oslash$  & $\bullet$  & $\bullet$  & $\otimes$ \\
Blockcerts    & $\otimes$  & $\bullet$ & $\bullet$  & $\bullet$  & $\bullet$  & $\bullet$  & $\bullet$ \\
BLOCK.CO      & $\bullet$  & $\bullet$ & $\bullet$  & $\otimes$  & $\bullet$  & $\bullet$  & $\otimes$ \\
SMART DIPLOMA & $\otimes$  & $\bullet$ & $\bullet$  & $\otimes$  & $\bullet$  & $\bullet$  & $\otimes$ \\
CVTRUST       & $\otimes$  & $\otimes$ & $\bullet$  & $\oslash$  & $\bullet$  & $\bullet$  & $\oslash$ \\
CVSS          & $\bullet$  & $\bullet$ & $\bullet$  & $\bullet$  & $\bullet$  & $\bullet$  & $\otimes$ \\
OUR SYSTEM    & $\bullet$  & $\bullet$ & $\bullet$  & $\bullet$  & $\bullet$  & $\bullet$  & $\bullet$ \\ \hline
$\oslash$= Partially Provided&$\bullet$= Provided    & $\otimes$= Unprovided  &   &   &   &   &     \\ \hline
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!htbp] \small
\centering
\caption{Transaction Times and Costs.}
\label{table:Transaction Times and Costs.}

\begin{tabular}{|l|c|}
\hline
Total Number of Transactions       & 219              \\ \hline
Total Confirmation Time (MM: SS)   & 17:32            \\ \hline
Average Confirmation Time (MM: SS) & 0.24             \\ \hline
Total Transactions Fee (Ether)     & 0.76703077 Ether \\ \hline
Average  Transactions Fee (Ether)  & 0.01091671 Ether \\ \hline
Total Transactions Fee (USD)       & \$657.409294     \\ \hline
Average  Transactions Fee (USD)    & \$6.15745258     \\ \hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!htbp] \small
\centering
\caption{Financial Comparison of CVSS and Our System.}
\label{tab:Financial Comparison of CVSS and Our System.}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|}
\cline{2-3}
                                                                             & \textbf{CVSS} & \textbf{Our System} \\ \hline
\multicolumn{1}{|l|}{\textbf{Contract Creation Cost}}                        & \$19                                  & \$10.76                                     \\ \hline
\multicolumn{1}{|l|}{\textbf{Number of Transactions}}                        & 60                                    & 219                                         \\ \hline
\multicolumn{1}{|l|}{\textbf{Transaction Cost}}                              & \$0.15                                & \$6.16                                      \\ \hline
\multicolumn{1}{|l|}{\textbf{Average Transaction Confirmation Time (mm:ss)}} & 00:60                                 & 00:24                                       \\ \hline
\multicolumn{1}{|l|}{\textbf{Total Transactions Confirmations Time (mm:ss)}} & 05:00                                 & 17:32                                       \\ \hline
\end{tabular}%
%}
\end{table}


\begin{table}[!htbp] \small
\centering
\caption{Different Blockchain Platforms and Their Characteristics.}
\label{table:Different Blockchain Platforms and Their Characteristics.}
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Blockchain Platform}} & \textbf{Network Permission} & \textbf{Smart Contract Support} \\ \hline
Bitcoin     & Permissionless              & No  \\ \hline
Ethereum    & Permissionless              & Yes \\ \hline
Zcash       & Permissionless              & No  \\ \hline
Litecoin    & Permissionless              & No  \\ \hline
Dash        & Permissionless              & No  \\ \hline
Peercoin    & Permissionless              & No  \\ \hline
Ripple      & Permissionless  (controlled) & No  \\ \hline
Monero      & Permissionless              & No  \\ \hline
MultiChain  & Permissionled               & No  \\ \hline
Hyperledger & Permissionled               & Yes \\ \hline
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
